In industrial embedded software, are some compilation errors easier to localize and fix than others?

Industrial embedded systems often require specialized hardware. However, software engineers have access to such domain-specific hardware only at the continuous integration (CI) stage and have to use simulated hardware otherwise. This results in a higher proportion of compilation errors at the CI stage than in other types of systems, warranting a deeper study. To this end, we create a CI diagnostics solution called ``Shadow Job'' that analyzes our industrial CI system. We collected over 40000 builds from 4 projects from the product source code and categorized the compilation errors into 14 error types, showing that the five most common ones comprise 89 % of all compilation errors. Additionally, we analyze the resolution time, size, and distance for each error type, to see if different types of compilation errors are easier to localize or repair than others. Our results show that the resolution time, size, and distance are independent of each other. Our research also provides insights into the human effort required to fix the most common industrial compilation errors. We also identify the most promising directions for future research on fault localization.

==> references.tex <==
@article{abrahamsson2017agile,
  author       = {Pekka Abrahamsson and
                  Outi Salo and
                  Jussi Ronkainen and
                  Juhani Warsta},
  title        = {Agile Software Development Methods: {Review} and analysis},
  journal      = {CoRR},
  volume       = {abs/1709.08439},
  year         = {2017},
  url          = {http://arxiv.org/abs/1709.08439},
  eprinttype    = {arXiv},
  eprint       = {1709.08439},
  timestamp    = {Mon, 13 Aug 2018 16:48:55 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1709-08439.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{chen2015continuous,
  author       = {Lianping Chen},
  title        = {Continuous Delivery: {Huge} Benefits, but Challenges Too},
  journal      = {{IEEE} Softw.},
  volume       = {32},
  number       = {2},
  pages        = {50--54},
  year         = {2015},
  url          = {https://doi.org/10.1109/MS.2015.27},
  doi          = {10.1109/MS.2015.27},
  timestamp    = {Mon, 08 Jun 2020 22:31:00 +0200},
  biburl       = {https://dblp.org/rec/journals/software/Chen15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{fu2022prevalence,
  author       = {Han Fu and
                  Sigrid Eldh and
                  Kristian Wiklund and
                  Andreas Ermedahl and
                  Cyrille Artho},
  title        = {Prevalence of continuous integration failures in industrial systems
                  with hardware-in-the-loop testing},
  booktitle    = {{IEEE} International Symposium on Software Reliability Engineering
                  Workshops, {ISSRE} 2022 - Workshops, Charlotte, NC, USA, October 31
                  - Nov. 3, 2022},
  pages        = {61--66},
  publisher    = {{IEEE}},
  year         = {2022},
  url          = {https://doi.org/10.1109/ISSREW55968.2022.00040},
  doi          = {10.1109/ISSREW55968.2022.00040},
  timestamp    = {Sun, 12 Nov 2023 02:12:28 +0100},
  biburl       = {https://dblp.org/rec/conf/issre/FuEWEA22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{antinyan2014identifying,
  author       = {Vard Antinyan and
                  Miroslaw Staron and
                  Wilhelm Meding and
                  Per {\"{O}}sterstr{\"{o}}m and
                  Erik Wikstrom and
                  Johan Wranker and
                  Anders Henriksson and
                  J{\"{o}}rgen Hansson},
  editor       = {Serge Demeyer and
                  Dave W. Binkley and
                  Filippo Ricca},
  title        = {Identifying risky areas of software code in {Agile/Lean} software development: {An} industrial experience report},
  booktitle    = {2014 Software Evolution Week - {IEEE} Conference on Software Maintenance,
                  Reengineering, and Reverse Engineering, {CSMR-WCRE} 2014, Antwerp,
                  Belgium, February 3-6, 2014},
  pages        = {154--163},
  publisher    = {{IEEE} Computer Society},
  year         = {2014},
  url          = {https://doi.org/10.1109/CSMR-WCRE.2014.6747165},
  doi          = {10.1109/CSMR-WCRE.2014.6747165},
  timestamp    = {Fri, 24 Mar 2023 00:02:40 +0100},
  biburl       = {https://dblp.org/rec/conf/csmr/AntinyanSMOWWHH14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{jonsson2013increasing,
  author       = {Leif Jonsson},
  editor       = {David Notkin and
                  Betty H. C. Cheng and
                  Klaus Pohl},
  title        = {Increasing anomaly handling efficiency in large organizations using
                  applied machine learning},
  booktitle    = {35th International Conference on Software Engineering, {ICSE} '13,
                  San Francisco, CA, USA, May 18-26, 2013},
  pages        = {1361--1364},
  publisher    = {{IEEE} Computer Society},
  year         = {2013},
  url          = {https://doi.org/10.1109/ICSE.2013.6606717},
  doi          = {10.1109/ICSE.2013.6606717},
  timestamp    = {Thu, 23 Mar 2023 23:58:06 +0100},
  biburl       = {https://dblp.org/rec/conf/icse/Jonsson04.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{kerzazi2014factors,
  author       = {Noureddine Kerzazi and
                  Foutse Khomh},
  editor       = {Maurizio Morisio and
                  Tore Dyb{\aa} and
                  Marco Torchiano},
  title        = {Factors impacting rapid releases: an industrial case study},
  booktitle    = {2014 {ACM-IEEE} International Symposium on Empirical Software Engineering
                  and Measurement, {ESEM} '14, Torino, Italy, September 18-19, 2014},
  pages        = {61:1--61:8},
  publisher    = {{ACM}},
  year         = {2014},
  url          = {https://doi.org/10.1145/2652524.2652589},
  doi          = {10.1145/2652524.2652589},
  timestamp    = {Tue, 06 Nov 2018 16:57:26 +0100},
  biburl       = {https://dblp.org/rec/conf/esem/KerzaziK14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{wong2016survey,
  author       = {W. Eric Wong and
                  Ruizhi Gao and
                  Yihao Li and
                  Rui Abreu and
                  Franz Wotawa},
  title        = {A Survey on Software Fault Localization},
  journal      = {{IEEE} Trans. Software Eng.},
  volume       = {42},
  number       = {8},
  pages        = {707--740},
  year         = {2016},
  url          = {https://doi.org/10.1109/TSE.2016.2521368},
  doi          = {10.1109/TSE.2016.2521368},
  timestamp    = {Tue, 13 Apr 2021 13:32:33 +0200},
  biburl       = {https://dblp.org/rec/journals/tse/WongGLAW16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{planning2002economic,
  title={The economic impacts of inadequate infrastructure for software testing},
  author={Planning, Strategic},
  journal={National Institute of Standards and Technology},
  volume={1},
  year={2002}
}

@inproceedings{hilton2016usage,
  author       = {Michael Hilton and
                  Timothy Tunnell and
                  Kai Huang and
                  Darko Marinov and
                  Danny Dig},
  editor       = {David Lo and
                  Sven Apel and
                  Sarfraz Khurshid},
  title        = {Usage, costs, and benefits of continuous integration in open-source
                  projects},
  booktitle    = {Proceedings of the 31st {IEEE/ACM} International Conference on Automated
                  Software Engineering, {ASE} 2016, Singapore, September 3-7, 2016},
  pages        = {426--437},
  publisher    = {{ACM}},
  year         = {2016},
  url          = {https://doi.org/10.1145/2970276.2970358},
  doi          = {10.1145/2970276.2970358},
  timestamp    = {Sat, 30 Sep 2023 09:51:40 +0200},
  biburl       = {https://dblp.org/rec/conf/kbse/HiltonTHMD16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{vasilescu2015quality,
  author       = {Bogdan Vasilescu and
                  Yue Yu and
                  Huaimin Wang and
                  Premkumar T. Devanbu and
                  Vladimir Filkov},
  editor       = {Elisabetta Di Nitto and
                  Mark Harman and
                  Patrick Heymans},
  title        = {Quality and productivity outcomes relating to continuous integration in {GitHub}},
  booktitle    = {Proceedings of the 2015 10th Joint Meeting on Foundations of Software
                  Engineering, {ESEC/FSE} 2015, Bergamo, Italy, August 30 - September
                  4, 2015},
  pages        = {805--816},
  publisher    = {{ACM}},
  year         = {2015},
  url          = {https://doi.org/10.1145/2786805.2786850},
  doi          = {10.1145/2786805.2786850},
  timestamp    = {Sun, 25 Oct 2020 23:14:01 +0100},
  biburl       = {https://dblp.org/rec/conf/sigsoft/VasilescuYWDF15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{vassallo2017tale,
  author       = {Carmine Vassallo and
                  Gerald Schermann and
                  Fiorella Zampetti and
                  Daniele Romano and
                  Philipp Leitner and
                  Andy Zaidman and
                  Massimiliano Di Penta and
                  Sebastiano Panichella},
  title        = {At tale of {CI} Build Failures: {An} Open Source and a Financial Organization
                  Perspective},
  booktitle    = {2017 {IEEE} International Conference on Software Maintenance and Evolution,
                  {ICSME} 2017, Shanghai, China, September 17-22, 2017},
  pages        = {183--193},
  publisher    = {{IEEE} Computer Society},
  year         = {2017},
  url          = {https://doi.org/10.1109/ICSME.2017.67},
  doi          = {10.1109/ICSME.2017.67},
  timestamp    = {Fri, 24 Mar 2023 00:04:10 +0100},
  biburl       = {https://dblp.org/rec/conf/icsm/VassalloSZRLZPP17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{beller2017oops,
  author       = {Moritz Beller and
                  Georgios Gousios and
                  Andy Zaidman},
  editor       = {Jes{\'{u}}s M. Gonz{\'{a}}lez{-}Barahona and
                  Abram Hindle and
                  Lin Tan},
  title        = {Oops, my tests broke the build: an explorative analysis of {Travis}
                  {CI} with {GitHub}},
  booktitle    = {Proceedings of the 14th International Conference on Mining Software
                  Repositories, {MSR} 2017, Buenos Aires, Argentina, May 20-28, 2017},
  pages        = {356--367},
  publisher    = {{IEEE} Computer Society},
  year         = {2017},
  url          = {https://doi.org/10.1109/MSR.2017.62},
  doi          = {10.1109/MSR.2017.62},
  timestamp    = {Thu, 23 Mar 2023 23:57:40 +0100},
  biburl       = {https://dblp.org/rec/conf/msr/BellerGZ17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{garousi2017test,
  author       = {Vahid Garousi and
                  Frank Elberzhager},
  title        = {Test Automation: Not Just for Test Execution},
  journal      = {{IEEE} Softw.},
  volume       = {34},
  number       = {2},
  pages        = {90--96},
  year         = {2017},
  url          = {https://doi.org/10.1109/MS.2017.34},
  doi          = {10.1109/MS.2017.34},
  timestamp    = {Mon, 08 Jun 2020 22:30:50 +0200},
  biburl       = {https://dblp.org/rec/journals/software/GarousiE17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{stolberg2009enabling,
  author       = {Sean Stolberg},
  editor       = {Yael Dubinsky and
                  Tore Dyb{\aa} and
                  Steve Adolph and
                  Ahmed Samy Sidky},
  title        = {Enabling Agile Testing through Continuous Integration},
  booktitle    = {2009 Agile Conference, Chicago, IL, USA, 24-28 August 2009},
  pages        = {369--374},
  publisher    = {{IEEE} Computer Society},
  year         = {2009},
  url          = {https://doi.org/10.1109/AGILE.2009.16},
  doi          = {10.1109/AGILE.2009.16},
  timestamp    = {Fri, 24 Mar 2023 00:05:03 +0100},
  biburl       = {https://dblp.org/rec/conf/agiledc/Stolberg09.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{zhang2019large,
  author       = {Chen Zhang and
                  Bihuan Chen and
                  Linlin Chen and
                  Xin Peng and
                  Wenyun Zhao},
  editor       = {Marlon Dumas and
                  Dietmar Pfahl and
                  Sven Apel and
                  Alessandra Russo},
  title        = {A large-scale empirical study of compiler errors in continuous integration},
  booktitle    = {Proceedings of the {ACM} Joint Meeting on European Software Engineering
                  Conference and Symposium on the Foundations of Software Engineering,
                  {ESEC/SIGSOFT} {FSE} 2019, Tallinn, Estonia, August 26-30, 2019},
  pages        = {176--187},
  publisher    = {{ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1145/3338906.3338917},
  doi          = {10.1145/3338906.3338917},
  timestamp    = {Sat, 30 Sep 2023 09:56:36 +0200},
  biburl       = {https://dblp.org/rec/conf/sigsoft/Zhang0C0Z19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{becker2019compiler,
  author       = {Brett A. Becker and
                  Paul Denny and
                  Raymond Pettit and
                  Durell Bouchard and
                  Dennis J. Bouvier and
                  Brian Harrington and
                  Amir Kamil and
                  Amey Karkare and
                  Chris McDonald and
                  Peter{-}Michael Osera and
                  Janice L. Pearce and
                  James Prather},
  editor       = {Bruce Scharlau and
                  Roger McDermott and
                  Arnold Pears and
                  Mihaela Sabin},
  title        = {Compiler Error Messages Considered Unhelpful: The Landscape of Text-Based
                  Programming Error Message Research},
  booktitle    = {Proceedings of the Working Group Reports on Innovation and Technology
                  in Computer Science Education, ITiCSE-WGR 2019, Aberdeen, Scotland
                  Uk, July 15-17, 2019},
  pages        = {177--210},
  publisher    = {{ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1145/3344429.3372508},
  doi          = {10.1145/3344429.3372508},
  timestamp    = {Sun, 26 Nov 2023 13:55:41 +0100},
  biburl       = {https://dblp.org/rec/conf/iticse/BeckerDPBB0KKMO19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{rosen1965pufft,
  author       = {Saul Rosen and
                  Robert A. Spurgeon and
                  Joel K. Donnelly},
  title        = {{PUFFT} - The {PURDUE} University fast {FORTRAN} translator},
  journal      = {Commun. {ACM}},
  volume       = {8},
  number       = {11},
  pages        = {661--666},
  year         = {1965},
  url          = {https://doi.org/10.1145/365660.365671},
  doi          = {10.1145/365660.365671},
  timestamp    = {Wed, 14 Nov 2018 10:22:34 +0100},
  biburl       = {https://dblp.org/rec/journals/cacm/RosenSD65.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{traver2010compiler,
  author       = {V. Javier Traver},
  title        = {On Compiler Error Messages: What They \emph{say} and What They \emph{mean}},
  journal      = {Adv. Hum. Comput. Interact.},
  volume       = {2010},
  pages        = {602570:1--602570:26},
  year         = {2010},
  url          = {https://doi.org/10.1155/2010/602570},
  doi          = {10.1155/2010/602570},
  timestamp    = {Fri, 09 Apr 2021 18:28:41 +0200},
  biburl       = {https://dblp.org/rec/journals/ahci/Traver10.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{seo2014programmers,
  author       = {Hyunmin Seo and
                  Caitlin Sadowski and
                  Sebastian G. Elbaum and
                  Edward Aftandilian and
                  Robert W. Bowdidge},
  editor       = {Pankaj Jalote and
                  Lionel C. Briand and
                  Andr{\'{e}} van der Hoek},
  title        = {Programmers' build errors: a case study (at {Google})},
  booktitle    = {36th International Conference on Software Engineering, {ICSE} '14,
                  Hyderabad, India - May 31 - June 07, 2014},
  pages        = {724--734},
  publisher    = {{ACM}},
  year         = {2014},
  url          = {https://doi.org/10.1145/2568225.2568255},
  doi          = {10.1145/2568225.2568255},
  timestamp    = {Tue, 06 Nov 2018 11:06:55 +0100},
  biburl       = {https://dblp.org/rec/conf/icse/SeoSEAB14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{barrak2021builds,
  author       = {Amine Barrak and
                  Ellis E. Eghan and
                  Bram Adams and
                  Foutse Khomh},
  title        = {Why do builds fail? - {A} conceptual replication study},
  journal      = {J. Syst. Softw.},
  volume       = {177},
  pages        = {110939},
  year         = {2021},
  url          = {https://doi.org/10.1016/j.jss.2021.110939},
  doi          = {10.1016/J.JSS.2021.110939},
  timestamp    = {Sat, 09 Apr 2022 12:28:16 +0200},
  biburl       = {https://dblp.org/rec/journals/jss/BarrakEAK21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{silva2023factors,
  author       = {Gustavo Silva and
                  Carla I. M. Bezerra and
                  Anderson G. Uch{\^{o}}a and
                  Ivan Machado},
  title        = {What Factors Affect the Build Failures Correction Time? {A} Multi-Project
                  Study},
  booktitle    = {Proceedings of the 17th Brazilian Symposium on Software Components,
                  Architectures, and Reuse, {SBCARS} 2023, Campo Grande, Brazil, September
                  25-29, 2023},
  pages        = {41--50},
  publisher    = {{ACM}},
  year         = {2023},
  url          = {https://doi.org/10.1145/3622748.3622753},
  doi          = {10.1145/3622748.3622753},
  timestamp    = {Sat, 14 Oct 2023 20:13:00 +0200},
  biburl       = {https://dblp.org/rec/conf/sbcars/SilvaBUM23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{kerzazi2014automated,
  author       = {Noureddine Kerzazi and
                  Foutse Khomh and
                  Bram Adams},
  title        = {Why Do Automated Builds Break? An Empirical Study},
  booktitle    = {30th {IEEE} International Conference on Software Maintenance and Evolution,
                  Victoria, BC, Canada, September 29 - October 3, 2014},
  pages        = {41--50},
  publisher    = {{IEEE} Computer Society},
  year         = {2014},
  url          = {https://doi.org/10.1109/ICSME.2014.26},
  doi          = {10.1109/ICSME.2014.26},
  timestamp    = {Fri, 24 Mar 2023 00:04:11 +0100},
  biburl       = {https://dblp.org/rec/conf/icsm/KerzaziKA14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{fischer2020forgotten,
  author       = {Anders Fischer{-}Nielsen and
                  Zhoulai Fu and
                  Ting Su and
                  Andrzej Wasowski},
  editor       = {Gregg Rothermel and
                  Doo{-}Hwan Bae},
  title        = {The forgotten case of the dependency bugs: on the example of the robot
                  operating system},
  booktitle    = {{ICSE-SEIP} 2020: 42nd International Conference on Software Engineering,
                  Software Engineering in Practice, Seoul, South Korea, 27 June - 19
                  July, 2020},
  pages        = {21--30},
  publisher    = {{ACM}},
  year         = {2020},
  url          = {https://doi.org/10.1145/3377813.3381364},
  doi          = {10.1145/3377813.3381364},
  timestamp    = {Wed, 05 May 2021 12:03:29 +0200},
  biburl       = {https://dblp.org/rec/conf/icse/Fischer-Nielsen20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{khazem2018making,
  author       = {Kareem Khazem and
                  Earl T. Barr and
                  Petr Hosek},
  editor       = {Frank Tip and
                  Eric Bodden},
  title        = {Making data-driven porting decisions with {Tuscan}},
  booktitle    = {Proceedings of the 27th {ACM} {SIGSOFT} International Symposium on
                  Software Testing and Analysis, {ISSTA} 2018, Amsterdam, The Netherlands,
                  July 16-21, 2018},
  pages        = {276--286},
  publisher    = {{ACM}},
  year         = {2018},
  url          = {https://doi.org/10.1145/3213846.3213855},
  doi          = {10.1145/3213846.3213855},
  timestamp    = {Wed, 25 Sep 2019 18:08:21 +0200},
  biburl       = {https://dblp.org/rec/conf/issta/KhazemBH18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{zakaria2022mapping,
  author       = {Farid Zakaria and
                  Thomas R. W. Scogland and
                  Todd Gamblin and
                  Carlos Maltzahn},
  editor       = {Felix Wolf and
                  Sameer Shende and
                  Candace Culhane and
                  Sadaf R. Alam and
                  Heike Jagode},
  title        = {Mapping Out the {HPC} Dependency Chaos},
  booktitle    = {{SC22:} International Conference for High Performance Computing, Networking,
                  Storage and Analysis, Dallas, TX, USA, November 13-18, 2022},
  pages        = {34:1--34:12},
  publisher    = {{IEEE}},
  year         = {2022},
  url          = {https://doi.org/10.1109/SC41404.2022.00039},
  doi          = {10.1109/SC41404.2022.00039},
  timestamp    = {Wed, 24 May 2023 16:17:06 +0200},
  biburl       = {https://dblp.org/rec/conf/sc/ZakariaSGM22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{ratti2018conceptual,
author="Ratti, Nisha
and Kaur, Parminder",
editor="Bhatia, Sanjiv K.
and Mishra, Krishn K.
and Tiwari, Shailesh
and Singh, Vivek Kumar",
title="A Conceptual Framework for Analysing the Source Code Dependencies",
booktitle="Advances in Computer and Computational Sciences",
year="2018",
publisher="Springer Singapore",
address="Singapore",
pages="333--341",
isbn="978-981-10-3773-3"
}

@inproceedings{rodrigues2021clp,
  author       = {Kirk Rodrigues and
                  Yu Luo and
                  Ding Yuan},
  editor       = {Angela Demke Brown and
                  Jay R. Lorch},
  title        = {{CLP:} Efficient and Scalable Search on Compressed Text Logs},
  booktitle    = {15th {USENIX} Symposium on Operating Systems Design and Implementation,
                  {OSDI} 2021, July 14-16, 2021},
  pages        = {183--198},
  publisher    = {{USENIX} Association},
  year         = {2021},
  url          = {https://www.usenix.org/conference/osdi21/presentation/rodrigues},
  timestamp    = {Fri, 04 Nov 2022 08:36:22 +0100},
  biburl       = {https://dblp.org/rec/conf/osdi/RodriguesLY21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{dai2020logram,
  author       = {Hetong Dai and
                  Heng Li and
                  Che{-}Shao Chen and
                  Weiyi Shang and
                  Tse{-}Hsun Chen},
  title        = {Logram: Efficient Log Parsing Using $n$n-Gram Dictionaries},
  journal      = {{IEEE} Trans. Software Eng.},
  volume       = {48},
  number       = {3},
  pages        = {879--892},
  year         = {2022},
  url          = {https://doi.org/10.1109/TSE.2020.3007554},
  doi          = {10.1109/TSE.2020.3007554},
  timestamp    = {Fri, 01 Apr 2022 11:24:48 +0200},
  biburl       = {https://dblp.org/rec/journals/tse/DaiLCSC22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{du2017deeplog,
  author       = {Min Du and
                  Feifei Li and
                  Guineng Zheng and
                  Vivek Srikumar},
  editor       = {Bhavani Thuraisingham and
                  David Evans and
                  Tal Malkin and
                  Dongyan Xu},
  title        = {DeepLog: {Anomaly} Detection and Diagnosis from System Logs through
                  Deep Learning},
  booktitle    = {Proceedings of the 2017 {ACM} {SIGSAC} Conference on Computer and
                  Communications Security, {CCS} 2017, Dallas, TX, USA, October 30 -
                  November 03, 2017},
  pages        = {1285--1298},
  publisher    = {{ACM}},
  year         = {2017},
  url          = {https://doi.org/10.1145/3133956.3134015},
  doi          = {10.1145/3133956.3134015},
  timestamp    = {Tue, 07 Mar 2023 10:47:41 +0100},
  biburl       = {https://dblp.org/rec/conf/ccs/Du0ZS17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{zhu2019tools,
  author       = {Jieming Zhu and
                  Shilin He and
                  Jinyang Liu and
                  Pinjia He and
                  Qi Xie and
                  Zibin Zheng and
                  Michael R. Lyu},
  editor       = {Helen Sharp and
                  Mike Whalen},
  title        = {Tools and benchmarks for automated log parsing},
  booktitle    = {Proceedings of the 41st International Conference on Software Engineering:
                  Software Engineering in Practice, {ICSE} {(SEIP)} 2019, Montreal,
                  QC, Canada, May 25-31, 2019},
  pages        = {121--130},
  publisher    = {{IEEE} / {ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1109/ICSE-SEIP.2019.00021},
  doi          = {10.1109/ICSE-SEIP.2019.00021},
  timestamp    = {Sat, 09 Apr 2022 12:43:05 +0200},
  biburl       = {https://dblp.org/rec/conf/icse/ZhuHLHXZL19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{fu2014digging,
  author       = {Xiaoyu Fu and
                  Rui Ren and
                  Sally A. McKee and
                  Jianfeng Zhan and
                  Ninghui Sun},
  title        = {Digging deeper into cluster system logs for failure prediction and
                  root cause diagnosis},
  booktitle    = {2014 {IEEE} International Conference on Cluster Computing, {CLUSTER}
                  2014, Madrid, Spain, September 22-26, 2014},
  pages        = {103--112},
  publisher    = {{IEEE} Computer Society},
  year         = {2014},
  url          = {https://doi.org/10.1109/CLUSTER.2014.6968768},
  doi          = {10.1109/CLUSTER.2014.6968768},
  timestamp    = {Thu, 23 Mar 2023 23:59:40 +0100},
  biburl       = {https://dblp.org/rec/conf/cluster/FuRMZS14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{lou2010mining,
  author       = {Jian{-}Guang Lou and
                  Qiang Fu and
                  Shengqi Yang and
                  Jiang Li and
                  Bin Wu},
  editor       = {Bharat Rao and
                  Balaji Krishnapuram and
                  Andrew Tomkins and
                  Qiang Yang},
  title        = {Mining program workflow from interleaved traces},
  booktitle    = {Proceedings of the 16th {ACM} {SIGKDD} International Conference on
                  Knowledge Discovery and Data Mining, Washington, DC, USA, July 25-28,
                  2010},
  pages        = {613--622},
  publisher    = {{ACM}},
  year         = {2010},
  url          = {https://doi.org/10.1145/1835804.1835883},
  doi          = {10.1145/1835804.1835883},
  timestamp    = {Tue, 01 Sep 2020 18:32:37 +0200},
  biburl       = {https://dblp.org/rec/conf/kdd/LouFYLW10.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{zhou2018fault,
  author       = {Xiang Zhou and
                  Xin Peng and
                  Tao Xie and
                  Jun Sun and
                  Chao Ji and
                  Wenhai Li and
                  Dan Ding},
  title        = {Fault Analysis and Debugging of Microservice Systems: Industrial Survey,
                  Benchmark System, and Empirical Study},
  journal      = {{IEEE} Trans. Software Eng.},
  volume       = {47},
  number       = {2},
  pages        = {243--260},
  year         = {2021},
  url          = {https://doi.org/10.1109/TSE.2018.2887384},
  doi          = {10.1109/TSE.2018.2887384},
  timestamp    = {Fri, 05 Nov 2021 10:54:22 +0100},
  biburl       = {https://dblp.org/rec/journals/tse/ZhouPXSJLD21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{lin2016log,
  author       = {Qingwei Lin and
                  Hongyu Zhang and
                  Jian{-}Guang Lou and
                  Yu Zhang and
                  Xuewei Chen},
  editor       = {Laura K. Dillon and
                  Willem Visser and
                  Laurie A. Williams},
  title        = {Log clustering based problem identification for online service systems},
  booktitle    = {Proceedings of the 38th International Conference on Software Engineering,
                  {ICSE} 2016, Austin, TX, USA, May 14-22, 2016 - Companion Volume},
  pages        = {102--111},
  publisher    = {{ACM}},
  year         = {2016},
  url          = {https://doi.org/10.1145/2889160.2889232},
  doi          = {10.1145/2889160.2889232},
  timestamp    = {Tue, 10 Aug 2021 14:29:46 +0200},
  biburl       = {https://dblp.org/rec/conf/icse/LinZLZC16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{he2018identifying,
  author       = {Shilin He and
                  Qingwei Lin and
                  Jian{-}Guang Lou and
                  Hongyu Zhang and
                  Michael R. Lyu and
                  Dongmei Zhang},
  editor       = {Gary T. Leavens and
                  Alessandro Garcia and
                  Corina S. Pasareanu},
  title        = {Identifying impactful service system problems via log analysis},
  booktitle    = {Proceedings of the 2018 {ACM} Joint Meeting on European Software Engineering
                  Conference and Symposium on the Foundations of Software Engineering,
                  {ESEC/SIGSOFT} {FSE} 2018, Lake Buena Vista, FL, USA, November 04-09,
                  2018},
  pages        = {60--70},
  publisher    = {{ACM}},
  year         = {2018},
  url          = {https://doi.org/10.1145/3236024.3236083},
  doi          = {10.1145/3236024.3236083},
  timestamp    = {Wed, 22 Jun 2022 12:16:13 +0200},
  biburl       = {https://dblp.org/rec/conf/sigsoft/HeLLZLZ18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{zhang2021onion,
  author       = {Xu Zhang and
                  Yong Xu and
                  Si Qin and
                  Shilin He and
                  Bo Qiao and
                  Ze Li and
                  Hongyu Zhang and
                  Xukun Li and
                  Yingnong Dang and
                  Qingwei Lin and
                  Murali Chintalapati and
                  Saravanakumar Rajmohan and
                  Dongmei Zhang},
  editor       = {Diomidis Spinellis and
                  Georgios Gousios and
                  Marsha Chechik and
                  Massimiliano Di Penta},
  title        = {Onion: identifying incident-indicating logs for cloud systems},
  booktitle    = {{ESEC/FSE} 2021: 29th {ACM} Joint European Software Engineering Conference
                  and Symposium on the Foundations of Software Engineering, Athens,
                  Greece, August 23-28, 2021},
  pages        = {1253--1263},
  publisher    = {{ACM}},
  year         = {2021},
  url          = {https://doi.org/10.1145/3468264.3473919},
  doi          = {10.1145/3468264.3473919},
  timestamp    = {Wed, 11 Jan 2023 16:10:39 +0100},
  biburl       = {https://dblp.org/rec/conf/sigsoft/ZhangXQHQLZLDLC21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ziftci2017broke,
  author       = {Celal Ziftci and
                  Jim Reardon},
  title        = {Who Broke the Build? Automatically Identifying Changes That Induce
                  Test Failures in Continuous Integration at {Google} Scale},
  booktitle    = {39th {IEEE/ACM} International Conference on Software Engineering:
                  Software Engineering in Practice Track, {ICSE-SEIP} 2017, Buenos Aires,
                  Argentina, May 20-28, 2017},
  pages        = {113--122},
  publisher    = {{IEEE} Computer Society},
  year         = {2017},
  url          = {https://doi.org/10.1109/ICSE-SEIP.2017.13},
  doi          = {10.1109/ICSE-SEIP.2017.13},
  timestamp    = {Thu, 23 Mar 2023 23:58:07 +0100},
  biburl       = {https://dblp.org/rec/conf/icse/ZiftciR17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{hassan2006using,
  author       = {Ahmed E. Hassan and
                  Ken Zhang},
  title        = {Using Decision Trees to Predict the Certification Result of a Build},
  booktitle    = {21st {IEEE/ACM} International Conference on Automated Software Engineering
                  {(ASE} 2006), 18-22 September 2006, Tokyo, Japan},
  pages        = {189--198},
  publisher    = {{IEEE} Computer Society},
  year         = {2006},
  url          = {https://doi.org/10.1109/ASE.2006.72},
  doi          = {10.1109/ASE.2006.72},
  timestamp    = {Fri, 24 Mar 2023 00:02:36 +0100},
  biburl       = {https://dblp.org/rec/conf/kbse/HassanZ06.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{le2011genprog,
  author       = {Claire Le Goues and
                  ThanhVu Nguyen and
                  Stephanie Forrest and
                  Westley Weimer},
  title        = {GenProg: {A} Generic Method for Automatic Software Repair},
  journal      = {{IEEE} Trans. Software Eng.},
  volume       = {38},
  number       = {1},
  pages        = {54--72},
  year         = {2012},
  url          = {https://doi.org/10.1109/TSE.2011.104},
  doi          = {10.1109/TSE.2011.104},
  timestamp    = {Tue, 21 Mar 2023 21:12:41 +0100},
  biburl       = {https://dblp.org/rec/journals/tse/GouesNFW12.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{naitou2018toward,
  author       = {Keigo Naitou and
                  Akito Tanikado and
                  Shinsuke Matsumoto and
                  Yoshiki Higo and
                  Shinji Kusumoto and
                  Hiroyuki Kirinuki and
                  Toshiyuki Kurabayashi and
                  Haruto Tanno},
  editor       = {Foutse Khomh and
                  Chanchal K. Roy and
                  Janet Siegmund},
  title        = {Toward introducing automated program repair techniques to industrial
                  software development},
  booktitle    = {Proceedings of the 26th Conference on Program Comprehension, {ICPC}
                  2018, Gothenburg, Sweden, May 27-28, 2018},
  pages        = {332--335},
  publisher    = {{ACM}},
  year         = {2018},
  url          = {https://doi.org/10.1145/3196321.3196358},
  doi          = {10.1145/3196321.3196358},
  timestamp    = {Wed, 11 Aug 2021 11:51:24 +0200},
  biburl       = {https://dblp.org/rec/conf/iwpc/NaitouTMHKKKT18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{marginean2019sapfix,
  author       = {Alexandru Marginean and
                  Johannes Bader and
                  Satish Chandra and
                  Mark Harman and
                  Yue Jia and
                  Ke Mao and
                  Alexander Mols and
                  Andrew Scott},
  editor       = {Helen Sharp and
                  Mike Whalen},
  title        = {SapFix: automated end-to-end repair at scale},
  booktitle    = {Proceedings of the 41st International Conference on Software Engineering:
                  Software Engineering in Practice, {ICSE} {(SEIP)} 2019, Montreal,
                  QC, Canada, May 25-31, 2019},
  pages        = {269--278},
  publisher    = {{IEEE} / {ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1109/ICSE-SEIP.2019.00039},
  doi          = {10.1109/ICSE-SEIP.2019.00039},
  timestamp    = {Tue, 13 Dec 2022 09:59:50 +0100},
  biburl       = {https://dblp.org/rec/conf/icse/MargineanBCH0MM19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{bader2019getafix,
  author       = {Johannes Bader and
                  Andrew Scott and
                  Michael Pradel and
                  Satish Chandra},
  title        = {Getafix: learning to fix bugs automatically},
  journal      = {Proc. {ACM} Program. Lang.},
  volume       = {3},
  number       = {{OOPSLA}},
  pages        = {159:1--159:27},
  year         = {2019},
  url          = {https://doi.org/10.1145/3360585},
  doi          = {10.1145/3360585},
  timestamp    = {Tue, 13 Dec 2022 09:59:49 +0100},
  biburl       = {https://dblp.org/rec/journals/pacmpl/BaderSP019.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{mesbah2019deepdelta,
  author       = {Ali Mesbah and
                  Andrew Rice and
                  Emily Johnston and
                  Nick Glorioso and
                  Edward Aftandilian},
  editor       = {Marlon Dumas and
                  Dietmar Pfahl and
                  Sven Apel and
                  Alessandra Russo},
  title        = {DeepDelta: learning to repair compilation errors},
  booktitle    = {Proceedings of the {ACM} Joint Meeting on European Software Engineering
                  Conference and Symposium on the Foundations of Software Engineering,
                  {ESEC/SIGSOFT} {FSE} 2019, Tallinn, Estonia, August 26-30, 2019},
  pages        = {925--936},
  publisher    = {{ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1145/3338906.3340455},
  doi          = {10.1145/3338906.3340455},
  timestamp    = {Tue, 01 Feb 2022 10:45:16 +0100},
  biburl       = {https://dblp.org/rec/conf/sigsoft/0001RJGA19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{gupta2017deepfix,
  author       = {Rahul Gupta and
                  Soham Pal and
                  Aditya Kanade and
                  Shirish K. Shevade},
  editor       = {Satinder Singh and
                  Shaul Markovitch},
  title        = {DeepFix: Fixing Common {C} Language Errors by Deep Learning},
  booktitle    = {Proceedings of the Thirty-First {AAAI} Conference on Artificial Intelligence,
                  February 4-9, 2017, San Francisco, California, {USA}},
  pages        = {1345--1351},
  publisher    = {{AAAI} Press},
  year         = {2017},
  url          = {http://aaai.org/ocs/index.php/AAAI/AAAI17/paper/view/14603},
  timestamp    = {Tue, 19 Apr 2022 16:03:28 +0200},
  biburl       = {https://dblp.org/rec/conf/aaai/GuptaPKS17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ahmed2018compilation,
  author       = {Umair Z. Ahmed and
                  Pawan Kumar and
                  Amey Karkare and
                  Purushottam Kar and
                  Sumit Gulwani},
  editor       = {Patricia Lago and
                  Michal Young},
  title        = {Compilation error repair: for the student programs, from the student
                  programs},
  booktitle    = {Proceedings of the 40th International Conference on Software Engineering:
                  Software Engineering Education and Training, {ICSE} {(SEET)} 2018,
                  Gothenburg, Sweden, May 27 - June 03, 2018},
  pages        = {78--87},
  publisher    = {{ACM}},
  year         = {2018},
  url          = {https://doi.org/10.1145/3183377.3183383},
  doi          = {10.1145/3183377.3183383},
  timestamp    = {Tue, 10 Aug 2021 14:29:45 +0200},
  biburl       = {https://dblp.org/rec/conf/icse/AhmedKKKG18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{xia2023keep,
  author       = {Chunqiu Steven Xia and
                  Lingming Zhang},
  title        = {Keep the Conversation Going: Fixing 162 out of 337 bugs for {\textdollar}0.42
                  each using {ChatGPT}},
  journal      = {CoRR},
  volume       = {abs/2304.00385},
  year         = {2023},
  url          = {https://doi.org/10.48550/arXiv.2304.00385},
  doi          = {10.48550/arXiv.2304.00385},
  eprinttype    = {arXiv},
  eprint       = {2304.00385},
  timestamp    = {Mon, 17 Apr 2023 15:20:10 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2304-00385.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{cohen2013applied,
  title={Applied multiple regression/correlation analysis for the behavioral sciences},
  author={Rutherford, Andrew},
  journal={British Journal of Mathematical \& Statistical Psychology},
  volume={56},
  pages={185},
  year={2003},
  publisher={British Psychological Society}
}

@INPROCEEDINGS{khandelwal2017enhancement,
  author={Khandelwal, Harita and Mankodi, Parthesh and Prajapati, Ritesh},
  booktitle={2017 International conference of Electronics, Communication and Aerospace Technology (ICECA)}, 
  title={Enhancement of automation testing system using {Yocto} project}, 
  year={2017},
  volume={1},
  number={},
  pages={697-700},
  doi={10.1109/ICECA.2017.8203630}}


@inproceedings{lundberg2017unified,
  author       = {Scott M. Lundberg and
                  Su{-}In Lee},
  editor       = {Isabelle Guyon and
                  Ulrike von Luxburg and
                  Samy Bengio and
                  Hanna M. Wallach and
                  Rob Fergus and
                  S. V. N. Vishwanathan and
                  Roman Garnett},
  title        = {A Unified Approach to Interpreting Model Predictions},
  booktitle    = {Advances in Neural Information Processing Systems 30: Annual Conference
                  on Neural Information Processing Systems 2017, December 4-9, 2017,
                  Long Beach, CA, {USA}},
  pages        = {4765--4774},
  year         = {2017},
  url          = {https://proceedings.neurips.cc/paper/2017/hash/8a20a8621978632d76c43dfd28b67767-Abstract.html},
  timestamp    = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/LundbergL17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}
